Weightless: Lossy Weight Encoding For Deep Neural Network Compression

The large memory requirements of deep neural networks limit their deployment and adoption on many devices. Model compression methods effectively reduce the memory requirements of these models, usually through applying transformations such as weight pruning or quantization. In this paper, we present a novel scheme for lossy weight encoding which complements conventional compression techniques. The encoding is based on the Bloomier filter, a probabilistic data structure that can save space at the cost of introducing random errors. Leveraging the ability of neural networks to tolerate these imperfections and by re-training around the errors, the proposed technique, Weightless, can compress DNN weights by up to 496x with the same model accuracy. This results in up to a 1.51x improvement over the state-of-the-art.

==> Makefile <==
# WARNING: DO NOT ADD CUSTOM BUILD COMMANDS TO THIS FILE.
#   This makefile is only provided as a courtesy shortcut for Linux users.
#		Using other toolchains, it is not used at all, so any additional custom
#   commands will not be executed, breaking those builds.


MAIN=ms
BIB=ml
FILES=conclusion.tex \
            context.tex \
          evaluation.tex \
            introduction.tex \
            method.tex
LIBS=iclr2018_conference.sty

${MAIN}.pdf: ${LIBS} ${MAIN}.tex ${FILES} ${MAIN}.bbl
	pdflatex ${MAIN}.tex
	pdflatex ${MAIN}.tex

${MAIN}.bbl: ${BIB}.bib ${MAIN}.aux
	bibtex ${MAIN}

${MAIN}.aux: ${MAIN}.tex
	pdflatex ${MAIN}.tex

clean:
	rm -f ${MAIN}.aux ${MAIN}.fdb_latexmk ${MAIN}.fls ${MAIN}.log ${MAIN}.pdf ${MAIN}.synctex.gz ${MAIN}.bbl ${MAIN}.blg

